PointFlow: Flowing Semantics Through Points for Aerial Image Segmentation

Aerial Image Segmentation is a particular semantic segmentation problem and has several challenging characteristics that general semantic segmentation does not have. There are two critical issues: The one is an extremely foreground-background imbalanced distribution, and the other is multiple small objects along with the complex background. Such problems make the recent dense affinity context modeling perform poorly even compared with baselines due to over-introduced background context. To handle these problems, we propose a point-wise affinity propagation module based on the Feature Pyramid Network (FPN) framework, named PointFlow. Rather than dense affinity learning, a sparse affinity map is generated upon selected points between the adjacent features, which reduces the noise introduced by the background while keeping efficiency. In particular, we design a dual point matcher to select points from the salient area and object boundaries, respectively. Experimental results on three different aerial segmentation datasets suggest that the proposed method is more effective and efficient than state-of-the-art general semantic segmentation methods. Especially, our methods achieve the best speed and accuracy trade-off on three aerial benchmarks. Further experiments on three general semantic segmentation datasets prove the generality of our method. Code will be provided in (https: //github.com/lxtGH/PFSegNets).

==> 0abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract} 
%The ABSTRACT is here 
% Need to rewrite 
%Aerial Image Segmentation is a particular semantic segmentation problem. It contains several challenging aspects that general semantic segmentation does not have. Two important issues are foreground-background imbalance and multiple small objects. To solve these problems, we propose PointFlow to better balance both foreground object contexts and semantic gap between resolution and semantics at the same time. Rather than dense affinity learning, a point-wised affinity map is estimated by selecting key points between the feature pyramids which reduce the noise introduced by the background while keeping efficiency. In particular, we design a dual point matcher to select semantic points in a complementary manner. Our proposed module is lightweight and can be adapted into various network architectures with significant gains. The experimental results using three different aerial segmentation datasets suggest that the proposed method is superior to the state-of-the-art general semantic segmentation methods while having the computation efficiency. Further experiments on three general semantic segmentation datasets prove the generality of our method. Both code and model will be available for further research.

% Aerial Image Segmentation is a particular semantic segmentation problem and has several unique challenging aspects that general semantic segmentation does not have. Two important issues are foreground-background imbalance and multiple small objects in the scene. Such problems make the recent dense affinity context modeling perform badly even compared with baselines due to over-introduced background context. To handle these problems, we propose a point-wised affinity propagation module, named PointFlow based on the FPN framework. Rather than dense affinity learning, a point-wised affinity map is estimated by selecting key points between the adjacent features which reduce the noise introduced by the background while keeping efficiency. In particular, we design a dual point matcher to select points from salient area and object boundaries respectively. The former samples salient points while the latter samples for object details. The experimental results using three different aerial segmentation datasets suggest that the proposed method is superior to the state-of-the-art general semantic segmentation methods while having the computation efficiency. Especially, our methods achieve the best speed and accuracy trade-off on three aerial benchmarks. Further experiments on three general semantic segmentation datasets prove the generality of our method. Both code and models will be available for further research.
%\textbf{Two critical issues are foreground-background imbalance and multiple small objects in the scene. } 

Aerial Image Segmentation is a particular semantic segmentation problem and has several challenging characteristics that general semantic segmentation does not have. There are two critical issues: The one is an extremely foreground-background imbalanced distribution, and the other is multiple small objects along with the complex background. Such problems make the recent dense affinity context modeling perform poorly even compared with baselines due to over-introduced background context. To handle these problems, we propose a point-wise affinity propagation module based on the Feature Pyramid Network(FPN) framework, named PointFlow. Rather than dense affinity learning, a sparse affinity map is generated upon selected points between the adjacent features, which reduces the noise introduced by the background while keeping efficiency. In particular, we design a dual point matcher to select points from the salient area and object boundaries, respectively. Experimental results on three different aerial segmentation datasets suggest that the proposed method is more effective and efficient than state-of-the-art general semantic segmentation methods. Especially, our methods achieve the best speed and accuracy trade-off on three aerial benchmarks. Further experiments on three general semantic segmentation datasets prove the generality of our method. Both code and models will be available for further research.
\end{abstract}
